Fiducial cross-section measurements of the production of a prompt photon in association with a top-quark pair at $\sqrt{s}=13$ TeV with the ATLAS detector at the LHC

The cross sections for top-quark pair production in association with a photon are measured in a fiducial volume with the ATLAS detector at a centre-of-mass energy of 13 TeV. Results are presented using proton-proton collision data collected by the LHC during 2015 and 2016, amounting to a total of 36.1 fb$^{-1}$. This also presents the first $t\bar{t}\gamma$ cross-section measurements performed in the dilepton channels. Exactly one photon is required to have $p_{\text{T}} > 20$ GeV and be isolated based on track and calorimeter information. At least two (four) jets are required in the dilepton (single-lepton) channels, with at least one jet originating from a $b$-quark. Two separate neural network algorithms are used to help reduce the impact backgrounds play in the final measurements. The Prompt Photon Tagger is trained on information from energy deposits in the calorimeters to distinguish prompt photons from hadronic fake photons. The output of this neural network is fed into the Event-level Discriminator that uses event information to classify signal from the sum of all backgrounds. A maximum likelihood fit is performed on the output of the Event-level Discriminator to determine the fiducial cross section of the signal process. The fiducial cross section for the single-lepton and dilepton channel are measured to be $521 \pm 9 \text{(stat.)} \pm 41 \text{(sys.)}$ fb and $69 \pm 3 \text{(stat.)} \pm 4\text{(sys.)}$ fb, respectively. In total, eight cross-section measurements are performed and all agree with theoretical next-to-leading-order predictions.

==> Title/Title_German.tex <==
\begin{titlepage}
\begin{center}
\begin{otherlanguage}{ngerman}
% Upper part of the page. The '~' is needed because \\
% only works if a paragraph has started.
%\includegraphics[width=0.15\textwidth]{./logo}~\\[1cm]

%\textsc{\LARGE University of Beer}\\[1.5cm]

%\textsc{\Large Final year project}\\[0.5cm]

% Title
\HRule \\[0.4cm]
{\Large \bfseries \TITLE \\[0.4cm] }

\HRule \\[1.5cm]
{\large
Dissertation\\[1.0cm]
zur Erlangung des mathematisch-naturwissenschaftlichen Doktorgrades\\
\glqq Doctor rerum naturalium\grqq\\
der Georg-August-Universit\"at G\"ottingen\\[1.0cm]
im Promotionsprogramm ProPhys\\
der Georg-August University School of Science (GAUSS)\\[2.0cm]
vorgelegt von\\[1.0cm]
\AUTHOR \\[0.5cm]
aus \COUNTRY \\[2.0cm]


% Author and supervisor
%\begin{minipage}{0.4\textwidth}
%\begin{flushleft} \large
%\emph{Author:}\\
%John \textsc{Smith}
%\end{flushleft}
%\end{minipage}
%\begin{minipage}{0.4\textwidth}
%\begin{flushright} \large
%\emph{Supervisor:} \\
%Dr.~Mark \textsc{Brown}
%\end{flushright}
%\end{minipage}

\vfill
G\"ottingen, 2018
}
% Bottom of the page
%{\large \today}
\end{otherlanguage}
\end{center}

\end{titlepage}


==> Title/Title_back_german.tex <==
\begin{otherlanguage}{ngerman}
\thispagestyle{empty}
{\small
\vfill
\noindent
\underline{Betreuungsausschuss}\\[0.2cm]
Prof. Dr. Arnulf Quadt \\
Prof. Dr. Stan Lai\\[1.0cm]

\noindent
\underline{Mitglieder der Pr\"ufungskommission:}\\[0.2cm]
\begin{tabular}{ll}
Referent: & Prof. Dr. Arnulf Quadt \\
{}&{\footnotesize II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen}\\[0.2cm]
Koreferent: &Prof. Dr. Stan Lai \\
{}&{\footnotesize II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen}\\[0.2cm]
\end{tabular}\\[1.0cm]


\noindent
\underline{Weitere Mitglieder der Pr\"ufungskommission:}\\[0.2cm]
Prof. Laura Covi, PhD \\
{\footnotesize Institut f\"ur Theoretische Physik, Georg-August-Universit\"at G\"ottingen}\\[0.2cm]
Prof. Dr. Ariane Frey \\
{\footnotesize II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen}\\[0.2cm]
Prof. Dr. Wolfram Kollatschny \\
{\footnotesize Institut f\"ur Astrophysik, Georg-August-Universit\"at G\"ottingen}\\[0.2cm]
Prof. Dr. Steffen Schumann \\
{\footnotesize Institut f\"ur Theoretische Physik, Georg-August-Universit\"at G\"ottingen}\\[0.2cm]
}
Tag der m\"undlichen Pr\"ufung: \\[1.0cm] % Do NOT insert a date here! Will be done by the examination office

\noindent
%Referenz: II.Physik-UniG\"o-Diss-2015/XX % Do NOT put a reference. This is not allowed!

\clearpage
\end{otherlanguage}
